Quantum Field Theories Coupled to Supergravity: AdS/CFT and Local Couplings

This article is based on my PhD thesis and covers the following topics: Holographic meson spectra in a dilaton flow background, the mixed Coulomb-Higgs branch in terms of instantons on D7 branes, and a dual description of heavy-light mesons. Moreover, in a second part the conformal anomaly of four dimensional supersymmetric quantum field theories coupled to classical N=1 supergravity is explored in a superfield formulation. The complete basis for the anomaly and consistency conditions, which arise from cohomological considerations, are given. Possible implications for an extension of Zamolodchikov's c-theorem to four dimensional supersymmetric quantum field theories are discussed.

==> chapters/0-i-dedication.tex <==

\vspace*{\stretch{1}}
\begin{flushright}
\begin{minipage}{10cm}
\begin{center}
\EPSinclude[width=10cm]{calista-coarse}\\[10ex]
%\UNLESSHYPER{\EPSinclude[width=10cm]{calista}}
%\EPSinclude[width=10cm]{calista}\\[10ex]
Dedicated to a true explorer
\end{center}
\end{minipage}
\end{flushright}
\vspace*{\stretch{1}}

==> chapters/0-ii-zusammenfassung.tex <==
\Chapter{Zusammenfassung}
%\pdfbookmark[1]{Zusammenfassung}{toc}
%\markboth{Zusammenfassung}{Zusammenfassung}
\begin{otherlanguage*}{ngerman}
Diese Dissertation ist der Untersuchung des Zusammenspiels von
supersymmetrischen Yang--Mills-Theorien (\acro{SYM}) und
Supergravitationstheorien (\acro{SUGRA}) gewidmet. Das Thema wird von zwei
Seiten beleuchtet:

Zun\"achst vom Standpunkt der \adscft\ Korrespondenz, die die Kopplung
zwischen vierdimensionaler superkonformer $\cN=4$ \acro{SYM}-Theorie
und zehndimensionaler Typ \acro{IIB} \acro{SUGRA} \emph{holographisch}
realisiert.  Um zu Theorien zu gelangen, die gr\"o\ss{}ere
\"Ahnlichkeit mit Quantenchromodynamik (\acro{QCD}) aufweisen, werden
fundamentale Felder mit Hilfe von D7\NB-Branen in die Korrespondenz
eingef\"uhrt und nicht-triviale Hintergrundkonfigurationen betrachtet.
Insbesondere werden Supergravitationsl\"osungen verwendet, die nur
noch asymptotisch die anti-de~Sitter-Geo\-me\-trie an\-n\"ah\-ern, was
Supersymmetrie bricht und die Beschreibung von spontaner chiraler
Symmetriebrechung erm\"oglicht. Das Mesonspektrum wird berechnet und
die Existenz einer zugeh\"origen Goldstone-Mode nachgewiesen sowie das
nicht Auftreten der Entartung bei Mesonen hoher radialer Anregung.
Dar\"uberhinaus werden Instantonkonfigurationen auf den D7\NB-Branen
untersucht, die zu einer Beschreibung des \emph{Higgs branch} der
dualen Feldtheorie f\"uhren.  Im Anschluss wird eine holographische
Beschreibung von \emph{heavy-light} Mesonen entwickelt, die sich aus
Quarks mit gro\ss{}em Massenunterschied zusammensetzen, was die
Behandlung von B\NB-Mesonen erm\"oglicht.

Als zweite Zugang zum Thema wird die Technik der sogenannten
ortsabh\"angigen (auch: \glqq lokalen\grqq) Kopplungen gew\"ahlt, bei
der die Kopplungskonstanten zu externen Quellen erweitert werden, was
die Untersuchung der konformen Anomalie von Quantenfeldtheorien, die
an einen klassischen Gravitationshintergrund gekoppelt werden,
erm\"oglicht.  Diese Technik wird auf die Superfeldbeschreibung
minimaler $\cN=1$ Supergravitation ausgedehnt, eine Basis f\"ur die
Anomalie angegeben und die Konsistenzbedingungen, die im Rahmen von
Kohomologiebetrachtungen auftreten, berechnet.  M\"ogliche
Implikationen f\"ur eine Erweiterung von Zamolodchikovs $c$-Theorem
auf vierdimensionale supersymmetrische Quantenfeldtheorien werden
diskutiert.
\end{otherlanguage*}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/diss/jo-diss"
%%% ispell-local-dictionary: "de"
%%% End: 





==> chapters/0-iii-abstract.tex <==
\begin{savequote}[\savequotewidth]
Who is General Failure and what did he do to my thesis?
\qauthor{author unknown (due to technical problems)}
\end{savequote}


%\ifBeautifulForm
\Chapter{Abstract}
%\else
%\begin{center}\textbf{Abstract}\end{center}\medskip
%\small
%\fi
%
This dissertation is devoted to the investigation of the interplay of
supersymmetric Yang--Mills theories (\acro{SYM}) and supergravity
(\acro{SUGRA}). The topic is studied from two points of view:

Firstly from the point of view of \adscftcorr, which realises the
coupling of four dimensional superconformal $\cN=4$ \acro{SYM} theory
and ten dimensional type \acro{IIB} \acro{SUGRA} in a
\emph{holographic} way.  In order to arrive at theories that resemble
quantum chromodynamics (\acro{QCD}) more closely, fundamental fields
are introduced using probe D7\NB-branes and non-trivial background
configuration are considered.  In particular supergravity solutions
that are only asymptotically anti-de~Sitter and break supersymmetry
are used. This allows the description of spontaneous chiral symmetry
breaking.  The meson spectrum is calculated and the existence of an
associated Goldstone mode is demonstrated. Moreover it is shown that
highly radially excited mesons are not degenerate.  Additionally
instanton configurations on the D7\NB-branes are investigated, which
lead to a holographic description of the dual field theory's
\emph{Higgs branch}.  Finally a holographic description of heavy-light
mesons is developed, which are mesons consisting of quarks with a
large mass difference, such that a treatment of B~mesons can be
achieved.

The second approach to the topic of this thesis is the technique of
so-called space-time dependent couplings (also known as ``local
couplings''), where coupling constants are promoted to external
sources.  This allows to explore the conformal anomaly of quantum
field theories coupled to a classical gravity background.  The
technique is extended to the superfield description of $\cN=1$
supergravity, a complete basis for the anomaly is given and the
consistency conditions that arise from a cohomological treatment are
calculated.  Possible implications for an extension of Zamolodchikov's
$c$\NB-theorem to four dimensional supersymmetric quantum field
theories are discussed.
%\ifBeautifulForm\else
%\normalsize
%\fi



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/diss/jo-diss"
%%% ispell-local-dictionary: "british"
%%% End: 


% LocalWords:  de


==> chapters/0-iv-preface.tex <==
\begin{savequote}[\savequotewidth]
  Success is the ability to go from one failure to another with no
  loss of enthusiasm.  
  \qauthor{Sir Winston Churchill} % (1874 - 1965)
\end{savequote}

\Chapter{Preface}

The work described in this thesis was carried out in collaboration
with Dr.~Johanna Erdmenger, Dr.~Zachary Guralnik and Dr.~Nick Evans.
This thesis covers the work presented in the following publications 
\cite{Erdmenger:2006bg,Apreda:2006ie,Erdmenger:2005bj,Grosse:2005}.

\begin{itemize}
\item  J.~Erdmenger, N.~Evans, J.G.,
       ``Heavy-Light Mesons from the \AdS/\linebreak[0]\acro{CFT}\ Correspondence,''
      \acro{JHEP} {\bf 0701}, 098 (2007)
      [\href{http://www.arxiv.org/abs/hep-th/0605241}{hep-th/0605241}].

\item R.~Apreda, J.~Erdmenger, N.~Evans, J.G., Z.~Guralnik,
      ``Instantons on D7\NB-brane probes and \adscft\ with flavour,''
      Fortsch.\ Phys.\  {\bf 54}, 266 (2006)
      %[arXiv:hep-th/0601130]
      [\href{http://www.arxiv.org/abs/hep-th/0601130}{hep-th/0601130}].

\item J.~Erdmenger, J.G., Z.~Guralnik,
      ``Spectral flow on the Higgs branch and \AdS/\acro{CFT} duality,''
      \acro{JHEP} {\bf 0506}, 052 (2005) 
      [\href{http://www.arxiv.org/abs/hep-th/0502224}{hep-th/0502224}].

\item J.G., ``MathPSfrag: Creating Publication-Quality Labels in
      Mathematica Plots,''
      submitted to Computer Physics Communications,
      \href{http://www.arxiv.org/abs/cs.GR/0510087}{cs.GR/0510087}.
\end{itemize}

Moreover the results of Chapter~\ref{ch:dilatondriven}, which
constitute independent work, have been presented in a talk at the
``XVI.~Workshop Beyond The Standard Model,'' Bad Honnef, March 8--11,
2004.

No claims to originality are made for the content of Chapters
\ref{ch:adscft-overview}, \ref{ch:flavour}, \ref{ch:sugra-overview}
and \ref{ch:local-couplings}, which were compiled
using a variety of sources.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/diss/jo-diss"
%%% ispell-local-dictionary: "british"
%%% End: 





% LocalWords:  Guralnik th Apreda Fortsch Honnef


==> chapters/A-determinant.tex <==

\Chapter{Determinant Expansion}
While most complicated backgrounds require working in the linearised
approximation (that is expansion to quadratic order of the \acro{DBI} action,
see sec.~\ref{sec:quaddbi}), for the vacuum solution there are occasions where
a full expansion of the determinant in the \acro{DBI} action is needed.
Since in string/M theory there is at most an eleven-dimensional metric, 
this can be easily done using a computer. However symbolic algebra programs
like \textsc{Mathematica}\textsuperscript{\textregistered} or 
\textsf{Maple}\textsuperscript{\textregistered} are sometimes not capable of
simplifying the result sufficiently well to obtain an expression suitable
for calculations by hand. In that case the following theorem, which is
probably well known in the mathematics literature (even though I could not
find it), can be useful as long as the metric is sufficiently simple.  
Since the formulation of the theorem is a bit hard to decode, 
studying the corollaries first might be helpful, in particular the last 
two corollaries, which are relevant for the pullback of a D7\NB-brane.

\begin{theorem}[Full Determinant Expansion] \mbox{}\\
Let $A,B$ be $N\times N$ matrices and $\one$ the corresponding unity matrix, then
it holds
\begin{gather}
  \det \left[ \one + AB \right] 
    = \det_{m,n} \left[ \delta_{mn} + A_{k_m m} B_{m k_n} \right] \quad \text{(no sum on m),} \label{eqn:det-theorem}
\end{gather}
where on the right hand side,  Einstein's convention is used on the indices $k_m$ after having evaluated the determinant in indices $m$ and $n$.

The right hand side may be formulated alternatively 
in the following manner:
\begin{gather}
  \det \left[ \one + AB \right] 
    = \sum_{k_1,\dots,k_N} \det \left[ \tfrac{1}{N} \delta_{mn} + A_{k_m m} B_{m k_n} \right] \quad \text{(no sum on m).}
\end{gather}
\end{theorem}

\begin{proof}
\begin{align}
  \text{LHS} 
    &= \det \left[ \one + AB \right] \notag\\ 
    &= \det \left[ \sum_{k} \left( \tfrac{1}{N} \delta_{mn} + A_{mk} B_{kn} \right) \right] \notag \\
    &= \sum_{\pi \in S_N} \sgn \pi \prod_m \sum_{k_m} \left( \tfrac{1}{N} \delta_{mn} + A_{m k_m} B_{k_m n} \right) \notag \\
    &= \sum_{k_1,\dots,k_N} \sum_{\pi \in S_N} \sgn \pi \prod_m  \left( \tfrac{1}{N} \delta_{m\pi(m)} + A_{m k_m} B_{k_m \pi(m)} \right) \\
    &= \sum_{k_1,\dots,k_N} \sum_{\pi \in S_N} \sgn \pi 
       \begin{aligned}[t] 
          \biggl[ & \prod_m  A_{m k_m} B_{k_m \pi(m)} +  \\
                 +& \prod_i  \tfrac{\delta_{i\pi(i)}}{N} \prod_{\substack{m\\m\neq i}}  A_{m k_m} B_{k_m \pi(m)} 
                 +  \dots  \biggr]  
       \end{aligned} \notag \\ 
    &= \sum_{k_1,\dots,k_N} \prod_m  A_{m k_m} \left[ \det B + \prod_i \tfrac{\delta_{i\pi(i)}}{N A_{m k_m}} \det \mathcal{B}_{ii} + \dots \right], \notag
\end{align}
where $\mathcal{B}_{ii}$ is the adjugate matrix corresponding to $B_{ii}$. 
\begin{align}
  \text{RHS} 
    &= \sum_{k_1,\dots,k_N} \det \left[ \tfrac{1}{N} \delta_{mn} + A_{k_m m} B_{m k_n} \right] \notag \\
    &= \sum_{k_1,\dots,k_N} \sum_{\pi \in S_N} \sgn \pi \prod_m  \left( \tfrac{1}{N} \delta_{m\pi(m)} + A_{k_m m} B_{m k_{\pi(m)}} \right)\notag\\
    &= \sum_{k_1,\dots,k_N} \sum_{\pi \in S_N} \sgn \pi \prod_m  \left( \tfrac{1}{N} \delta_{m\pi(m)} + A_{m k_m} B_{k_{\pi(m)} m} \right)\\
%
    &= \sum_{k_1,\dots,k_N} \sum_{\pi \in S_N} \sgn \pi 
       \begin{aligned}[t] 
          \biggl[ & \prod_m  A_{m k_m} B_{k_{\pi(m)} m} +  \\
                 +& \prod_i  \tfrac{\delta_{i\pi(i)}}{N} \prod_{\substack{m\\m\neq i}}  A_{m k_m} B_{k_{\pi(m)} m} 
                 +  \dots  \biggr]  
       \end{aligned} \notag\\ 
    &= \sum_{k_1,\dots,k_N} \prod_m  A_{m k_m} \left[ \det B + \prod_i \tfrac{\delta_{i\pi(i)}}{N A_{m k_m}} \det \mathcal{B}_{ii} + \dots \right]\notag\\
    &=  \text{LHS} %\tag*{$\blacksquare$}
\end{align}
\end{proof}

\begin{corollary}[Vector formulation] \mbox{}\\
%
For the matrices 
\begin{align}
  A &= (\vec{a}_1,\dots,\vec{a}_N), &
  B &= \smash{\begin{pmatrix}\vec{b}_1^T\\ \vdots \\ \vec{b}_N^T \end{pmatrix}}, 
\end{align}
theorem \eqref{eqn:det-theorem} reads
\begin{gather}
  \det \left[ \one + \sum_\lambda \vec{a}_\lambda \otimes \vec{b}_\lambda \right] 
    = \det \left[ \delta_{mn} + (\vec{a}_m)_{k_m} (\vec{b}_m)_{k_n} \right],
\end{gather}
where again Einstein's convention is used on $k_m$.
\end{corollary}

\begin{corollary}[Fewer vectors]  \mbox{}\\
For $\vec{a}_\lambda = \vec{b}_\lambda = 0 \quad \forall\; \lambda > L$ this is
\begin{align}
\begin{split}
  \det &\left[ \one + \sum_{\lambda=1}^L \vec{a}_\lambda \otimes \vec{b}_\lambda \right] \\
    &= \det \begin{pmatrix}
               \delta_{mn} + (\vec{a}_m)_{k_m} (\vec{b}_m)_{k_n} & \text{irrelevant} \\
               0 & \one_{N-L}
           \end{pmatrix} \\
    &= \det \left[ \delta_{\mu\nu} + (\vec{a}_\mu)_{k_\mu} (\vec{b}_\mu)_{k_\nu} \right],
\end{split}
\end{align}
with indices $\mu,\nu$ running from $1$ to $L$ and summation on indices $k_\mu.$ The right hand 
side may be evaluated using the following simple \textsc{Mathematica} script.
\begin{align}
\begin{split}
{\scriptstyle1}&\quad \mathtt{ rank = 4; \quad (* \text{ plug in appropriate value } *) }\\
{\scriptstyle2}&\quad \mathtt{ Expand\bigl[Det\bigl[Table\bigl[dummy[i][j],\; \{i,rank\},\; \{j,rank\} \bigr]\bigr]\bigr] \mathrel{/.} }\\
 &\quad \mathtt{ \qquad  dummy[x\_][y\_] \mathrel{:\!\to} KroneckerDelta[x,y] + \vectt{a}_x[x] \vectt{b}_y[y]; }\\
{\scriptstyle3}&\quad \mathtt{ result = (\% \mathrel{//.}  \vectt{a}_{i\_}[k\_] \vectt{b}_{j\_}[k\_] \to \vectt{a}_i \cdot \vectt{b}_j]) }
\end{split}
\end{align}
\end{corollary}

\begin{corollary}[D7 pullback for diagonal metric] \mbox{ } \\
For $L=2$ one obtains
\begin{align}
\begin{split}
  \det &\left[ \one + \vec{a}_1 \otimes \vec{b}_1 + \vec{a}_2 \otimes \vec{b}_2 \right] \\
    &= \det \begin{pmatrix}
          1+ (\vec{a}_1)_{k_1} (\vec{b}_1)_{k_1} &     (\vec{a}_1)_{k_1} (\vec{b}_1)_{k_2}  \\
          (\vec{a}_2)_{k_2} (\vec{b}_2)_{k_1}    & 1 + (\vec{a}_2)_{k_2} (\vec{b}_2)_{k_2} 
       \end{pmatrix} \\
    &= (1+\vec{a}_1\vec{b}_1)(1+\vec{a}_2\vec{b}_2)-(\vec{a}_2\vec{b}_1)(\vec{a}_1\vec{b}_2),
\end{split}
\end{align}
%
which for the vectors
\begin{align}
  (\vec{a}_1)_b &= G_{88} G^{bc} \partial_c z^8, & 
  (\vec{a}_2)_b &= G_{99} G^{bc} \partial_c z^9, \\ 
  (\vec{b}_1)_a &= \partial_a z^8, & 
  (\vec{b}_2)_a &= \partial_a z^9 
\end{align}
yields
\begin{align}
\begin{split}
  \det &\left[ \one + G_{88} G^{bc} \partial_c z^8 \partial_a z^8 + G_{99} G^{bc} \partial_c z^9 \partial_a z^9 \right] \\
    &= (1+G_{88} G^{bc} \partial_b z^8 \partial_c z^8 )(1+G_{99} G^{bc} \partial_b z^9 \partial_c z^9)\\
    &\phantom{=}- G_{88} G_{99} (G^{bc} \partial_b z^8 \partial_c z^9)^2.
\end{split}
\end{align}
\end{corollary}

\begin{corollary}[D7 pullback for block diagonal metric]\mbox{}\\
For a ten-dimensional metric of the form 
\begin{align}
  G_{AB} \,dX^A\, dX^B 
    =  \begin{pmatrix} dx^a dz^i \end{pmatrix}
       \begin{pmatrix} 
          g_{ab} & 0 \\
          0 & g_{ij}
       \end{pmatrix} 
       \begin{pmatrix} dx^b \\ dz^j \end{pmatrix}
\end{align}
with indices $a,b=0,\dots,7$ and $i,j=8,9,$ 
the determinant of an eight dimensional pullback with respect to 
the embedding $x^a = \xi^a, z^i = z^i(\xi^a)$ is given by
\begin{align}
\begin{split}
  \det & P[G_{AB}] \\
    &= \det \left\{ g_{ab} + g_{ij} \frac{\partial z^i}{\partial\xi^a} \frac{\partial z^j}{\partial\xi^b} \right\} \\
    &= \det g_{ab} \cdot \det \left\{ \one_8 + g_{ij} \partial_a z^i \partial_b z^j  g^{bc} \right\}\\
    &= \det g_{ab} \cdot \det \left[ \one + \sum_{\lambda=1}^4 \vec{a}_\lambda \otimes \vec{b}_\lambda \right]  
\end{split}
\end{align}
%  \det \left[ \one + \sum_\lambda \vec{a}_\lambda \otimes \vec{b}_\lambda \right] 
%    = \det \left[ \delta_{mn} + (\vec{a}_m)_{k_m} (\vec{b}_m)_{k_n} \right],
%
with the vectors  $\vec{a}_\lambda, \vec{b}_\lambda$ given by
\begin{align*}
  \vec{a}_1 &:= g_{88}\, (g)\cdot\vec{\nabla}z^8, & 
  \vec{b}_1 &:= \vec{\nabla}z^8, \\
  \vec{a}_2 &:= g_{89}\, (g)\cdot \vec{\nabla}z^8, & 
  \vec{b}_2 &:= \vec{\nabla}z^9, \\
  \vec{a}_3 &:= g_{98}\, (g)\cdot \vec{\nabla}z^9 
              = g_{98} / g_{88} \, \vec{a}_1, & 
  \vec{b}_3 &:= \vec{\nabla}z^8 = \vec{b}_1, \\
  \vec{a}_4 &:= g_{99}\, (g)\cdot \vec{\nabla}z^9 
              = g_{99} / g_{89} \,\vec{a}_2, & 
  \vec{b}_4 &:= \vec{\nabla}z^9 = \vec{b}_2,  
\end{align*}
where $(g)\cdot \vec{\nabla}$ denotes the matrix multiplication $g^{ab}\p_b$.
Using the theorem this may be expanded into $4!=24$ terms, which due to above
proportionality properties can be dramatically simplified, and one obtains
\begin{align}
\begin{split}
  \det P[G_{AB}] = \det g_{cd} \cdot \Bigl( 
         1 &+ g_{ij} \partial_a z^i \partial_b z^j g^{ab} \\&+ \det g_{ij} \cdot \det_{kl} \left\{ \partial_a z^k\partial_bz^l g^{ab} \right\} \Bigr),
\end{split}
\end{align}
where
\begin{align}
\begin{split}
 \det_{kl}&\left\{ \partial_a z^k\partial_b z^l g^{ab} \right\} \\
    &= (g^{ab} \partial_a z^8 \partial_b z^8)(g^{cd} \partial_c z^8 \partial_d z^8) - (g^{ab} \partial_a z^8 \partial_b z^9)^2.       
\end{split}
\end{align}
Note that no approximation has been used.
\end{corollary}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/diss/jo-diss"
%%% ispell-local-dictionary: "british"
%%% End: 



% LocalWords:  mn LHS mk RHS eqn det KroneckerDelta bc dX dx ij bz cd adjugate


==> chapters/B-walkerratum.tex <==
\Chapter{Mini-Erratum for ``Walk~through~Superspace''}

The following is a list of minor misprints I found in the second
revision (1998) of Buchbinder/Kuzenko's excellent book on supergravity
\cite{Buchbinder:1998qv}.  Since the second part of this thesis is based on
the definitions and conventions presented there, I would like to 
point out that at least those deviations from the book that are included below
are intentional.
In addition let me state, that I am aware of most of them
ranging from self-evident to trivial.  The format of this list is
``error'' $\mapsto$ ``correct''.
%
\begin{itemize}
\item \emph{p.~426, eq.~5.3.53} \\
  $\comm{\D_\ia}{\D_{\ib\db}} = \half \veps_{\ia\ib} T^\ic \D_{\ic \db} - \dots$ 
  $\mapsto$ 
  $\comm{\D_\ia}{\D_{\ib\db}} = \half \veps_{\ia\ib} T^\ic \D_{\ic \db} + \dots$\\
  \emph{Suggestion:} In the same equations, parenthesise according to\\
   $ i (\D_\ib R) \bM_{\da\db} $ and  $ i (\bD_\db \bR) M_{\ia\ib} $.
\item \emph{p.~427, sec.~5.3.7}\\
  ``unless $R\neq0$'' $\mapsto$ ``unless $R=0$''
\item \emph{p.~428, eq.~5.3.59}\\
  $T'_\ia = L T_\ia - \D'_\ia \ln L^4 \bar{L}^2 $ $\mapsto$
  $T'_\ia = L T_\ia + \D'_\ia \ln L^4 \bar{L}^2 $\\
  \emph{Suggestion:} Give the Weyl transformation behaviour of all
  non-minimal fields.
\item \emph{p.~443, eq.~5.5.6}\\
  $\comm{\D_\ia}{\bD_{\ib\db}}$ $\mapsto$ $\comm{\D_\ia}{\D_{\ib\db}}$ \\
  $\comm{\bD_\da}{\bD_{\ib\db}}$ $\mapsto$ $\comm{\bD_\da}{\D_{\ib\db}}$\\
  \emph{Suggestion:}  Again write 
  $i (\D_\ib R) \bM_{\da\db} $ and  $ i (\bD_\db \bR) M_{\ia\ib} $.
\item \emph{p.~444, eq.~5.5.9d}\\
  $\comm{\D^2}{\D_\da}$ $\mapsto$ $\comm{\D^2}{\bD_\da}$ \\
  $8 \bW_\da{}^{\dc\dd} M_{\dc\dd}$ $\mapsto$ $8 \bW_\da{}^{\dc\dd} \bM_{\dc\dd}$
\item \emph{p.~446, eq.~5.5.14}\\
  $G'_\ada = \e^{-(\sigma-\bsigma)/2}$ $\mapsto$ $G'_\ada = \e^{-(\sigma+\bsigma)/2}$
\item \emph{p.~461, eq.~5.6.57}\\
   $\tilde{\mathcal{E}}^{-1} = E^{-1} ( \sigma + \bsigma \dots)$
   $\mapsto$
   $\tilde{\mathcal{E}}^{-1} = E^{-1} ( 1+ \sigma + \bsigma \dots)$
\item \emph{p.~466, eq.~5.7.5}\\
   $\tilde\chi_{(\nabla)} = \e^{-i \mathbf{H}} \tilde\chi_{(\nabla)} $
   $\mapsto$
   $\tilde\chi_{(\nabla)} = \e^{-i \mathbf{H}} \chi_{(\nabla)} $\\
\item \emph{p.~472, above eq.~5.7.40}\\
   $\delta S = \int \dots {\displaystyle\frac{1}{R}} \bsigma \bT 
   \mapsto
   \delta S = \int \dots {\displaystyle\frac{1}{\bR}} \bsigma \bT
   $

\item \emph{p.~475, eq.~5.8.55}\\ 
  $-\quart \hat{E}^2 \varphi | = e^{-1/3} (B+\tfrac{2}{3}\dots)$ 
  $\mapsto$
  $-\quart \hat{E}^2 \varphi | = \tfrac{1}{3} e^{-1/3} (B+\tfrac{2}{3}\dots)$
\item \emph{p.~489, 2nd eq.}\\ 
   $(\bD - 4 R) \Lag$ $\mapsto$ $(\bD^2 - 4 R) \Lag$
\item \emph{p.~490, eq.~5.8.50}\\
   $-\quart \bD^2 \Lag_c$ $\mapsto$ $-\quart \D^2 \Lag_c$  
\item \emph{p.~541, 1st line}\\
   ``gravity action (6.6.1)'' $\mapsto$ ``gravity action (6.1.1)''
\item \emph{p.~542, eq.~6.6.22}\\
   $\D_\da \sigma = 0$ $\mapsto$ $\bD_\da\sigma=0$
\item \emph{p.~624, eq.~7.4.23}\\
   $(\bD^2-4R) \Omega = 0$ $\mapsto$ $(\D^2 -4\bR)\Omega = 0, (\bD_\da \Omega = 0)$
\end{itemize}

%
%\Section*{Trivial}
%\comment{Remove this Section from the thesis}
%\begin{itemize}
%\item \emph{p.~441, last paragraph}\\
%  ``he role'' $\mapsto$ ``the role''
%\item \emph{p.~460, below eq. 5.6.52}\\
%   ``To complete out'' $\mapsto$ ``To complete our''
%\item \emph{p.~472, below eq.~5.7.41}\\
%   \emph{Suggestion:} Define $\stackrel{\leftrightarrow}{\D}_\ada 
%                      := \D_\ada - \stackrel{\leftarrow}{\D}_\ada$
%\end{itemize}
%

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/diss/jo-diss"
%%% ispell-local-dictionary: "british"
%%% End: 

% LocalWords:  Superspace Buchbinder Kuzenko's nd


==> chapters/Vitae.tex <==
\begin{savequote}[\savequotewidth]
  I was born not knowing and have had only a little time to change
  that here and there.  
  \qauthor{Richard Feynman} 
  % (1918 - 1988), Letter to Armando Garcia J, December 11, 1985}
\end{savequote}

\Chapter{Curriculum Vit\ae}

\Section*{Personal Details}
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}>{\sffamily}llc>{\sffamily}ll}
Name                 & Johannes Gro\ss{}e && Nationality & German \\
Date of Birth        & March 31, 1978     && Parents     & Annelie Gro\ss{}e\\
Place of Birth       & Berlin             &&             & Eckhardt Blankertz \\
Marital Status       & Married, 1 child \\
\end{tabular*}

\Section*{Education}
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}>{\sffamily}lrp{80mm}}
Ph.D.             &  \llap{04.}2005 & Continued at \\ &&\textsl{Ludwig-Maximilians-Universit\"at~M\"unchen}\\
Ph.D.             &  \llap{04.}2003 & Started at \\ &&\textsl{Humboldt-Universit\"at zu Berlin}\\
Diplom            &  \llap{12.}2002 & Thesis on ``AdS/CFT Correspondence and Renormalization Group Flows'',
                                      117 pages, \acro{GPA}~1.0, Supervisor Prof.\ Dieter L\"ust,
                                      \textsl{Humboldt-Universit\"at zu Berlin}\\
Vordiplom         &  \llap{09.}1999 & \acro{GPA}~1.5, \textsl{Humboldt-Universit\"at zu Berlin} \\
A-Level           &            1997 & \acro{GPA}~1.0, \textsl{Lise-Meitner-Oberschule Berlin}\\
Grammar School    &            1990 & \textsl{Hermann-Hesse-Oberschule} \\
Primary School      &            1984 & \textsl{Adolf-Gla\ss{}brenner-Grundschule} 
\end{tabular*}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/diss/jo-diss"
%%% ispell-local-dictionary: "british"
%%% End: 

% LocalWords:  Vit llc Gro Annelie Eckhardt Blankertz lrp Ph Universit unchen
% LocalWords:  zu Diplom Renormalization Vordiplom Meitner Oberschule Gla
% LocalWords:  brenner Grundschule


==> chapters/preamble.tex <==
% preamble

%\usepackage{amsthm}
%\theoremstyle{definition}
%
%\usepackage[font={small}]{caption}
%\usepackage[ngerman,english]{babel}
%
%\newcommand{\horizrule}{\begin{center}\rule{5cm}{1pt}\end{center}}


%\setlength{\savequotewidth}{80mm}
%\usepackage{setspace}

% optische Randkorrektur mit sehr konservative Einstellungen:
%\ifpdf\usepackage[final,protrusion=compatibility,expansion=false]{microtype}\fi
%\ifpdf\usepackage[final,protrusion=true,expansion=false]{microtype}\fi

% --- tweak LaTeX's float placement algorithm ---
%\renewcommand{\topfraction}{1.0}
%\renewcommand{\textfraction}{0.0}
%\renewcommand{\floatpagefraction}{0.75}
%


% Andere wichtige Zeichen sind |\iff| $\iff$, |\implies| $\implies$
% und |\impliedby| $\impliedby$, die auch bereits die richtigen 
% Abst"ande verwenden.
% \DeclareMathOperator{\sdet}{sdet}
% \DeclareMathOperator{\arcoth}{arcoth}
% \DeclareMathOperator{\arccot}{arccot}
% \DeclareMathOperator{\sgn}{sgn}
% \DeclareMathOperator{\hyperFtwoone}{{}_2F_1}
% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}

% \newcommand{\mrlap}[1]{\rlap{$\displaystyle#1$}}
% \newcommand{\pfrac}[2]{\genfrac{(}{)}{}{}{#1}{#2}}
% \newcommand{\lieD}{\mathcal{L}}

% \newcommand{\vectt}[1]{\mathnormal{\vec{\,\mathtt{#1}}}}

% \newcommand{\vs}{\mathrel{\leftrightarrow}}
% \newcommand{\lvec}[1]{\stackrel{\leftarrow}{#1}}
% \newcommand{\lrvec}[1]{\stackrel{\leftrightarrow}{#1}}
% \newcommand{\iphi}{\mathrm{i}_\Phi}
% \newcommand{\covD}{\mathcal{D}}
% \newcommand{\cH}{\mathcal{H}}
% \newcommand{\cT}{\mathcal{T}}
% \newcommand{\bE}{\bar{E}}
% \newcommand{\bPhi}{\bar{\Phi}}
% \newcommand{\tE}{\tilde{E}}
% \newcommand{\tR}{\tilde{R}}
% \newcommand{\tmq}{\tilde{m}_q}
% \newcommand{\tmh}{\tilde{m}_H}
% \newcommand{\tml}{\tilde{m}_L}
% \newcommand{\tvphi}{\tilde{\vphi}}
% \newcommand{\bB}{\bar{B}}
% \newcommand{\bF}{\bar{F}}
% \newcommand{\bN}{\bar{N}}
% \newcommand{\gr}[1]{\mathrm{#1}} % group
% \newcommand{\mf}[1]{\mathrm{#1}} % manifold
% \newcommand{\al}[1]{\mathfrak{#1}} % algebra
% \newcommand{\UU}{\mathbb{U}}
% \newcommand{\bUU}{\bar{\mathbb{U}}}
% \newcommand{\TT}{\mathbb{T}}
% \newcommand{\bTT}{\bar{\mathbb{T}}}
% \newcommand{\WW}{\mathbb{W}}
% \newcommand{\bWW}{\bar{\mathbb{W}}}

% \providecommand{\href}[2]{#2}
% \providecommand{\texorpdfstring}[2]{#1}

% \hyphenation{con-ven-tion-al}
% \hyphenation{Gub-ser}
% \hyphenation{der-i-va-tion}
% \hyphenation{mes-on}  % Ja das trennt man wirklich so im Englischen!
% \hyphenation{mes-ons}
% \newcommand{\naive}{na\-\"{\i}ve}
% \newcommand{\role}{r\^{o}le}
% \newcommand{\emt}{en\-er\-gy-mo\-men\-tum tensor}

%\let\originalvec=\vec
%\renewcommand{\vec}[1]{{\originalvec{#1}\,}}
%\newcommand{\sqvec}[1]{\vec{#1}^2}
%\newcommand{\sqvec}[1]{\vec{#1}\,{}^2}
%\newcommand{\panti}{(anti\nobreakdash-)\linebreak[0]}

%\DeclareRobustCommand{\AdS}{\ifmmode\mf{AdS}\else\acro{AdS}\fi}
%\newcommand{\Afluct}{\mathcal{A}}
%\newcommand{\Ainst}{A^{\text{inst}}}
%\newcommand{\spinl}{\ensuremath{\ell}}
%\newcommand{\pfrac}[2]{\genfrac{(}{)}{}{}{#1}{#2}}  % fraction with parentheses
%\newcommand{\tpfrac}[2]{\genfrac{(}{)}{}{1}{#1}{#2}}% same but smaller

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: ~/diss/jo-diss.tex
%%% End: 


==> pictures/flow-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (flow-psfrag.eps). 
% psfrag replacement commands
\psfrag{AdS}{$\AdS_5$}
\psfrag{5}{}
\psfrag{D7}{D7}
\psfrag{3}{}
\psfrag{S}{$\mf{S}^3$}
\psfrag{r}{$r$}
\psfrag{r=m}[tr][tr]{$r=\tilde{m}_q$}


==> pictures/fluct-sols-psfrag.tex <==
% psfrag replacement commands
\psfrag{a1}[tc][tc][1][0]{$1$}
\psfrag{a2}[tc][tc][1][0]{$2$}
\psfrag{a3}[tc][tc][1][0]{$3$}
\psfrag{a4}[tc][tc][1][0]{$4$}
\psfrag{a5Lowe}[Bc][Bc][1][0]{}
\psfrag{a5}[tc][tc][1][0]{$5$}
\psfrag{fRho}[Bc][Bc][1][0]{$f(\rho )$}
\psfrag{Rho}[Bl][Bl][1][0]{$\rho $}

==> pictures/gubser-actions-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-actions-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a01}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.1}$}
\psfrag{a02}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.2}$}
\psfrag{a03000}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.3}$}
\psfrag{a04}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.4}$}
\psfrag{a05A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.5}$}
\psfrag{a05B}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.5}$}
\psfrag{a05}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.5}$}
\psfrag{a15A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.5}$}
\psfrag{a15}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-1.5}$}
\psfrag{a1A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.0}$}
\psfrag{a1}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-1.0}$}
\psfrag{mq}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{(2\pi\alpha')m_q}{r_0}}$}
\psfrag{S0Smq}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{E(m_q)-E(0)}$}\psfrag{PrecedA}[br][br][\psfragdefaultscale][0]{$\psfragmathstyle{\langle \bar{\psi}\psi\rangle >0}$}
\psfrag{Preced}[tr][tr][\psfragdefaultscale][0]{$\psfragmathstyle{\langle \bar{\psi}\psi\rangle <0}$}


==> pictures/gubser-gmor-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-gmor-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a01}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.1}$}
\psfrag{a02}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.2}$}
\psfrag{a03000}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.3}$}
\psfrag{a05}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.5}$}
\psfrag{a15}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.5}$}
\psfrag{a1}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.0}$}
\psfrag{a25}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{2.5}$}
\psfrag{a2}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{2.0}$}
\psfrag{a3}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{3.0}$}
\psfrag{m}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{(2\pi\alpha')m_q}{r_0}}$}
\psfrag{MTheta}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{M_{\pi}^2\, L^4}{r_0^2}}$}

==> pictures/gubser-highexcite-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-highexcite-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a10A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a10}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a15}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{15}$}
\psfrag{a20A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a20}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a25}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{25}$}
\psfrag{a30A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{30}$}
\psfrag{a30}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{30}$}
\psfrag{a40}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{40}$}
\psfrag{a50}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{50}$}
\psfrag{a5}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{5}$}
\psfrag{a60}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{60}$}
\psfrag{a70}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{70}$}
\psfrag{M}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{M}$}
\psfrag{n}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{n}$}

==> pictures/gubser-highexcite1-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-highexcite1-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a10A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a10}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a15}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{15}$}
\psfrag{a20A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a20}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a25}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{25}$}
\psfrag{a30A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{30}$}
\psfrag{a30}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{30}$}
\psfrag{a40}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{40}$}
\psfrag{a50}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{50}$}
\psfrag{a5}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{5}$}
\psfrag{a60}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{60}$}
\psfrag{a70}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{70}$}
\psfrag{MTheta}[bl][bl][\psfragdefaultscale][0]{$\psfragtextstyle{M_\pi, M_\sigma, M_{\text{KMMW}}}$}
\psfrag{n}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{n}$}

==> pictures/gubser-highexcite2-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-highexcite2-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a10}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a15}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{15}$}
\psfrag{a1A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1}$}
\psfrag{a1}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-1}$}
\psfrag{a20}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a25}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{25}$}
\psfrag{a2}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-2}$}
\psfrag{a30}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{30}$}
\psfrag{a3}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-3}$}
\psfrag{a5}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{5}$}
\psfrag{CDelta}[bc][bc][\psfragdefaultscale][0]{$\Delta M$}
\psfrag{MSigma}[cl][Bl][\psfragdefaultscale][0]{$\quad M_{\sigma }-M_{\text{KMMW}}$}
\psfrag{MTheta}[cl][tl][\psfragdefaultscale][0]{$\quad M_{\pi }-M_{\text{KMMW}}$}
\psfrag{n}[cl][cl][\psfragdefaultscale][0]{$n$}

==> pictures/gubser-lowmesons-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-lowmesons-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a05}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.5}$}
\psfrag{a15}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{1.5}$}
\psfrag{a1}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{1.0}$}
\psfrag{a25}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{2.5}$}
\psfrag{a2A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{2}$}
\psfrag{a2}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{2.0}$}
\psfrag{a3}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{3.0}$}
\psfrag{a4}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{4}$}
\psfrag{a6}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{6}$}
\psfrag{a8}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{8}$}
\psfrag{m}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{(2\pi\alpha')m_q}{r_0}}$}
\psfrag{MTheta}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{M_{\pi, \sigma, \rho }\,L^2}{r_0}}$}
\psfrag{pseudo}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\text{pseudoscalar}}$}
\psfrag{scalar}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\text{scalar}}$}
\psfrag{SUSY}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\text{SUSY}}$}
\psfrag{vector}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\text{vector}}$}

==> pictures/gubser-m-vs-c-linear-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-m-vs-c-linear-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a10}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a5}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{5}$}
\psfrag{a6A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{6}$}
\psfrag{a6}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{6}$}
\psfrag{a7A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{7}$}
\psfrag{a7}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{7}$}
\psfrag{a8A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{8}$}
\psfrag{a8}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{8}$}
\psfrag{a9}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{9}$}
\psfrag{c1}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{r_0^3}{c}}$}
\psfrag{m}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{(2\pi\alpha')m_q}{r_0}}$}

==> pictures/gubser-m-vs-c-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-m-vs-c-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a025}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.25}$}
\psfrag{a05}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.50}$}
\psfrag{a075}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.75}$}
\psfrag{a10}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a125}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.25}$}
\psfrag{a15}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.50}$}
\psfrag{a175}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.75}$}
\psfrag{a1}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.00}$}
\psfrag{a2}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{2}$}
\psfrag{a4}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{4}$}
\psfrag{a6}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{6}$}
\psfrag{a8}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{8}$}
\psfrag{c}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{c}{r_0^3}}$}
\psfrag{m}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{(2\pi\alpha')m_q}{r_0}}$}

==> pictures/gubser-negmass-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-negmass-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a05A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.5}$}
\psfrag{a05}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.5}$}
\psfrag{a10}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a1A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.0}$}
\psfrag{a1}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-1.0}$}
\psfrag{a2}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{2}$}
\psfrag{a4}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{4}$}
\psfrag{a6}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{6}$}
\psfrag{a8}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{8}$}
\psfrag{Sigma0}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{z_0(y)}{r_0}}$}
\psfrag{y}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{y}{r_0}}$}

==> pictures/gubser-vac-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-vac-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a05A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.5}$}
\psfrag{a05}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.5}$}
\psfrag{a15A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.5}$}
\psfrag{a15}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{1.5}$}
\psfrag{a1A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{1.0}$}
\psfrag{a1}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{1.0}$}
\psfrag{a25}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{2.5}$}
\psfrag{a2A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{2.0}$}
\psfrag{a2}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{2.0}$}
\psfrag{a3}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{3.0}$}
\psfrag{mq04c1}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\;m_q=0.4;\; c=1.479}$}
\psfrag{mq08c1}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\;m_q=0.8;\; c=1.183}$}
\psfrag{mq0c17}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\;m_q=0.0;\; c=1.765}$}
\psfrag{mq12c0}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\;m_q=1.2;\; c=0.929}$}
\psfrag{mq16c0}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\;m_q=1.6;\; c=0.737}$}
\psfrag{mq2c06}[cl][cl][\psfragdefaultscale][0]{$\psfragtextstyle{\;m_q=2.0;\; c=0.603}$}
\psfrag{Sigma0}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{z_0(y)}{r_0}}$}
\psfrag{y}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{y/r_0}$}

==> pictures/gubser-zeta5-far-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-zeta5-far-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a0001A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.001}$}
\psfrag{a0001}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.001}$}
\psfrag{a0002A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.002}$}
\psfrag{a0002}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.002}$}
\psfrag{a0003A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.003}$}
\psfrag{a0003}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.003}$}
\psfrag{a100}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{100}$}
\psfrag{a20}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a40}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{40}$}
\psfrag{a60}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{60}$}
\psfrag{a80}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{80}$}
\psfrag{y}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{y}$}
\psfrag{Zeta5y}[bc][tc][\psfragdefaultscale][0]{$\psfragmathstyle{\zeta^8(y)}$}

==> pictures/gubser-zeta5-middle-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-zeta5-middle-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a00025A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.0025}$}
\psfrag{a00025}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.0025}$}
\psfrag{a0005A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.005}$}
\psfrag{a0005}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.005}$}
\psfrag{a00075A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{0.0075}$}
\psfrag{a00075}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.0075}$}
\psfrag{a1}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{1}$}
\psfrag{a2}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{2}$}
\psfrag{a3}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{3}$}
\psfrag{a4}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{4}$}
\psfrag{a5}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{5}$}
\psfrag{y}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{y}$}
\psfrag{Zeta5y}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\zeta^8(y)}$}

==> pictures/gubser-zeta5-zoom-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (gubser-zeta5-zoom-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a0012}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.012}$}
\psfrag{a0014}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.014}$}
\psfrag{a0016}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.016}$}
\psfrag{a00180}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.018}$}
\psfrag{a002}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{0.020}$}
\psfrag{a066}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.66}$}
\psfrag{a068}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.68}$}
\psfrag{a072}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{-0.72}$}
\psfrag{y}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{y}$}
\psfrag{Zeta5y}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\zeta ^8(y)}$}

==> pictures/hl-ads-converge-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-ads-converge-psfrag.eps). 
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][1][0]{$0$}
\psfrag{a100a}[tc][tc][1][0]{$100$}
\psfrag{a1200000000a}[cr][cr][1][0]{$1.2$}
\psfrag{a1400000000a}[cr][cr][1][0]{$1.4$}
\psfrag{a16a}[cr][cr][1][0]{$1.6$}
\psfrag{a18a}[cr][cr][1][0]{$1.8$}
\psfrag{a1a}[bc][bc][1][0]{$1$}
\psfrag{a20a}[tc][tc][1][0]{$20$}
\psfrag{a22a}[cr][cr][1][0]{$2.2$}
\psfrag{a2400000000a}[cr][cr][1][0]{$2.4$}
\psfrag{a2a}[cr][cr][1][0]{$2$}
\psfrag{a40a}[tc][tc][1][0]{$40$}
\psfrag{a60a}[tc][tc][1][0]{$60$}
\psfrag{a80a}[tc][tc][1][0]{$80$}
\psfrag{aMHLmHa}[bc][bc][1][0]{$\displaystyle\frac{\tilde{M}_{HL}}{\tilde{m}_H}$}
\psfrag{aSpectrumfoa}[bc][bc][1][0]{}
\psfrag{aSqrtLambdaa}[cl][cl][1][0]{$\sqrt{\lambda }$}

==> pictures/hl-ads-gubser-comparison-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-ads-gubser-comparison-psfrag.eps). 
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][1][0]{$0$}
\psfrag{a100a}[tc][tc][1][0]{$100$}
\psfrag{a10a}[cr][cr][1][0]{$10$}
\psfrag{a15a}[cr][cr][1][0]{$15$}
\psfrag{a20Aa}[cr][cr][1][0]{$20$}
\psfrag{a20a}[tc][tc][1][0]{$20$}
\psfrag{a25a}[cr][cr][1][0]{$25$}
\psfrag{a30a}[cr][cr][1][0]{$30$}
\psfrag{a40a}[tc][tc][1][0]{$40$}
\psfrag{a5a}[cr][cr][1][0]{$5$}
\psfrag{a60a}[tc][tc][1][0]{$60$}
\psfrag{a80a}[tc][tc][1][0]{$80$}
\psfrag{aAdSGubserca}[bc][bc][1][0]{}
\psfrag{aSqrtLambdaAa}[bc][bc][1][0]{$\sqrt{\lambda } \left(\frac{M_{\text{HL}}}{m_H}-1\right)$}
\psfrag{aSqrtLambdaa}[cl][cl][1][0]{$\sqrt{\lambda }$}

==> pictures/hl-ads-linear-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-ads-linear-psfrag.eps). 
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][1][0]{$0$}
\psfrag{a100Aa}[cr][cr][1][0]{$100$}
\psfrag{a100a}[tc][tc][1][0]{$100$}
\psfrag{a120a}[cr][cr][1][0]{$120$}
\psfrag{a20Aa}[cr][cr][1][0]{$20$}
\psfrag{a20a}[tc][tc][1][0]{$20$}
\psfrag{a40Aa}[cr][cr][1][0]{$40$}
\psfrag{a40a}[tc][tc][1][0]{$40$}
\psfrag{a60Aa}[cr][cr][1][0]{$60$}
\psfrag{a60a}[tc][tc][1][0]{$60$}
\psfrag{a80Aa}[cr][cr][1][0]{$80$}
\psfrag{a80a}[tc][tc][1][0]{$80$}
\psfrag{aSpectrumfoa}[bc][bc][1][0]{}
\psfrag{aSqrtLambdaAa}[bc][bc][1][0]{$\displaystyle\frac{\sqrt{\lambda }\, \tilde{M}_{HL}}{\tilde{m}_H}$}
\psfrag{aSqrtLambdaa}[cl][cl][1][0]{$\sqrt{\lambda }$}

==> pictures/hl-ads-small-div-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-ads-small-div-psfrag.eps). 
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][1][0]{$0$}
\psfrag{a10a}[cr][cr][1][0]{$10$}
\psfrag{a15a}[cr][cr][1][0]{$15$}
\psfrag{a1a}[tc][tc][1][0]{$1$}
\psfrag{a20a}[cr][cr][1][0]{$20$}
\psfrag{a25a}[cr][cr][1][0]{$25$}
\psfrag{a2a}[tc][tc][1][0]{$2$}
\psfrag{a30a}[cr][cr][1][0]{$30$}
\psfrag{a3a}[tc][tc][1][0]{$3$}
\psfrag{a4a}[tc][tc][1][0]{$4$}
\psfrag{a5Aa}[cr][cr][1][0]{$5$}
\psfrag{a5a}[tc][tc][1][0]{$5$}
\psfrag{aMHLmHa}[bc][bc][1][0]{$\frac{M_{\text{HL}}}{m_H}$}
\psfrag{aSpectrumfoa}[bc][bc][1][0]{$\text{Spectrum for small $\lambda $}$}
\psfrag{aSqrtLambdaa}[cl][cl][1][0]{$\sqrt{\lambda }$}

==> pictures/hl-ads-small-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-ads-small-psfrag.eps). 
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][1][0]{$0$}
\psfrag{a10a}[cr][cr][1][0]{$10$}
\psfrag{a15a}[cr][cr][1][0]{$15$}
\psfrag{a1a}[tc][tc][1][0]{$1$}
\psfrag{a20a}[cr][cr][1][0]{$20$}
\psfrag{a25a}[cr][cr][1][0]{$25$}
\psfrag{a2a}[tc][tc][1][0]{$2$}
\psfrag{a30a}[cr][cr][1][0]{$30$}
\psfrag{a3a}[tc][tc][1][0]{$3$}
\psfrag{a4a}[tc][tc][1][0]{$4$}
\psfrag{a5Aa}[cr][cr][1][0]{$5$}
\psfrag{a5a}[tc][tc][1][0]{$5$}
\psfrag{aSpectrumfoa}[bc][bc][1][0]{}
\psfrag{aSqrtLambdaAa}[bc][bc][1][0]{$\displaystyle\frac{\sqrt{\lambda }\, \tilde{M}_{HL} }{\tilde{m}_H}$}
\psfrag{aSqrtLambdaa}[cl][cl][1][0]{$\sqrt{\lambda }$}

==> pictures/hl-adsprop-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-adsprop-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a10A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{10.0}$}
\psfrag{a10}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a125}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{12.5}$}
\psfrag{a15A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{15.0}$}
\psfrag{a15}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{15}$}
\psfrag{a20}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a25}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{2.5}$}
\psfrag{a5A}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{5.0}$}
\psfrag{a5}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{5}$}
\psfrag{a75}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{7.5}$}
\psfrag{MHLmH}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{M_{HL}}{m_H}}$}
\psfrag{n}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{n}$}

==> pictures/hl-cm-b-bstar-ratio-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-b-bstar-ratio-psfrag.eps). 
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][1][0]{$0$}
\psfrag{a100a}[tc][tc][1][0]{$100$}
\psfrag{a11a}[cr][cr][1][0]{$1.1$}
\psfrag{a1200000000a}[cr][cr][1][0]{$1.2$}
\psfrag{a13a}[cr][cr][1][0]{$1.3$}
\psfrag{a1400000000a}[cr][cr][1][0]{$1.4$}
\psfrag{a15a}[cr][cr][1][0]{$1.5$}
\psfrag{a1a}[bc][bc][1][0]{$1$}
\psfrag{a20a}[tc][tc][1][0]{$20$}
\psfrag{a40a}[tc][tc][1][0]{$40$}
\psfrag{a60a}[tc][tc][1][0]{$60$}
\psfrag{a80a}[tc][tc][1][0]{$80$}
\psfrag{aMSuperStara}[bc][bc][1][0]{$\frac{M_{B^*}}{M_B}$}
\psfrag{aSqrtLambdaa}[cl][cl][1][0]{$\sqrt{\lambda }$}

==> pictures/hl-cm-psfrag.tex <==
% -- content from the Prologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file. 
\providecommand{\psfragtextscale}{1}
\providecommand{\psfragmathscale}{\psfragtextscale}
\providecommand{\psfragnumericscale}{\psfragtextscale}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of Prologue option --

% psfrag replacement commands
\psfrag{a100}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{100}$}
\psfrag{a10}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a15}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{15}$}
\psfrag{a20A}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a20}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a25}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{25}$}
\psfrag{a30}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{30}$}
\psfrag{a40}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{40}$}
\psfrag{a5}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{5}$}
\psfrag{a60}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{60}$}
\psfrag{a80}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{80}$}
\psfrag{Consta}[bc][bc][\psfragtextscale][0]{}
\psfrag{MMeson}[bc][bc][\psfragmathscale][0]{$\psfragmathstyle{\tilde{M}_{HL}}$}
\psfrag{Mq}[cl][cl][\psfragmathscale][0]{$\psfragmathstyle{\tilde{m}_H}$}


==> pictures/hl-cm-scaled-psfrag.tex <==
% -- content from the Prologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file. 
\providecommand{\psfragtextscale}{1}
\providecommand{\psfragmathscale}{\psfragtextscale}
\providecommand{\psfragnumericscale}{\psfragtextscale}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of Prologue option --

% psfrag replacement commands
\psfrag{a10A}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a10}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a12}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{12}$}
\psfrag{a14}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{14}$}
\psfrag{a15}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{15}$}
\psfrag{a20}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a25}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{25}$}
\psfrag{a2}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{2}$}
\psfrag{a30}[tc][tc][\psfragnumericscale][0]{$\psfragnumericstyle{30}$}
\psfrag{a4}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{4}$}
\psfrag{a6}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{6}$}
\psfrag{a8}[cr][cr][\psfragnumericscale][0]{$\psfragnumericstyle{8}$}
\psfrag{Consta}[bc][bc][\psfragtextscale][0]{}
\psfrag{MMeson}[bc][bc][\psfragmathscale][0]{$\psfragmathstyle{\displaystyle\frac{\tilde{M}_{HL}}{\tilde{m}_H}}$}
\psfrag{Mq}[cl][cl][\psfragmathscale][0]{$\psfragmathstyle{\tilde{m}_H}$}


==> pictures/hl-cm-xmas-compare-lambda100-all-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-cm-xmas-compare-lambda100-all-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][\psfragdefaultscale][0]{$0$}
\psfrag{a10a}[tc][tc][\psfragdefaultscale][0]{$10$}
\psfrag{a15a}[tc][tc][\psfragdefaultscale][0]{$15$}
\psfrag{a1a}[cr][cr][\psfragdefaultscale][0]{$1$}
\psfrag{a20a}[tc][tc][\psfragdefaultscale][0]{$20$}
\psfrag{a25a}[tc][tc][\psfragdefaultscale][0]{$25$}
\psfrag{a2a}[cr][cr][\psfragdefaultscale][0]{$2$}
\psfrag{a30a}[tc][tc][\psfragdefaultscale][0]{$30$}
\psfrag{a3a}[cr][cr][\psfragdefaultscale][0]{$3$}
\psfrag{a4a}[cr][cr][\psfragdefaultscale][0]{$4$}
\psfrag{a5Aa}[cr][cr][\psfragdefaultscale][0]{$5$}
\psfrag{a5a}[tc][tc][\psfragdefaultscale][0]{$5$}
\psfrag{a6a}[cr][cr][\psfragdefaultscale][0]{$6$}
\psfrag{am1MHLmHa}[bc][bc][\psfragdefaultscale][0]{$\frac{M_{\text{HL}}}{m_H}-1$}
\psfrag{amHCLambdaba}[cl][cl][\psfragdefaultscale][0]{$\frac{m_H}{\Lambda _b}$}

==> pictures/hl-comparison-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-comparison-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][\psfragdefaultscale][0]{$0$}
\psfrag{a100a}[tc][tc][\psfragdefaultscale][0]{$100$}
\psfrag{a10a}[cr][cr][\psfragdefaultscale][0]{$10$}
\psfrag{a15a}[cr][cr][\psfragdefaultscale][0]{$15$}
\psfrag{a20Aa}[cr][cr][\psfragdefaultscale][0]{$20$}
\psfrag{a20a}[tc][tc][\psfragdefaultscale][0]{$20$}
\psfrag{a25a}[cr][cr][\psfragdefaultscale][0]{$25$}
\psfrag{a30a}[cr][cr][\psfragdefaultscale][0]{$30$}
\psfrag{a40a}[tc][tc][\psfragdefaultscale][0]{$40$}
\psfrag{a5a}[cr][cr][\psfragdefaultscale][0]{$5$}
\psfrag{a60a}[tc][tc][\psfragdefaultscale][0]{$60$}
\psfrag{a80a}[tc][tc][\psfragdefaultscale][0]{$80$}
\psfrag{aAdSCMcompaa}[bc][bc][\psfragdefaultscale][0]{}%{$\text{AdS/CM comparison for }m_H\text{=12.6305}$}
\psfrag{aSqrtLambdaAa}[bc][bc][\psfragdefaultscale][0]{$\sqrt{\lambda } \left(\frac{M_{\text{HL}}}{m_H}-1\right)$}
\psfrag{aSqrtLambdaa}[cl][cl][\psfragdefaultscale][0]{$\sqrt{\lambda }$}

==> pictures/hl-gubser-b-bstar-ratio-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-gubser-b-bstar-ratio-psfrag.eps). 
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][1][0]{$0$}
\psfrag{a100a}[tc][tc][1][0]{$100$}
\psfrag{a11a}[cr][cr][1][0]{$1.1$}
\psfrag{a1200000000a}[cr][cr][1][0]{$1.2$}
\psfrag{a13a}[cr][cr][1][0]{$1.3$}
\psfrag{a1400000000a}[cr][cr][1][0]{$1.4$}
\psfrag{a15a}[cr][cr][1][0]{$1.5$}
\psfrag{a1a}[bc][bc][1][0]{$1$}
\psfrag{a20a}[tc][tc][1][0]{$20$}
\psfrag{a40a}[tc][tc][1][0]{$40$}
\psfrag{a60a}[tc][tc][1][0]{$60$}
\psfrag{a80a}[tc][tc][1][0]{$80$}
\psfrag{aMSuperStara}[bc][bc][1][0]{$\frac{M_{B^*}}{M_B}$}
\psfrag{aSqrtLambdaa}[cl][cl][1][0]{$\sqrt{\lambda }$}

==> pictures/hl-gubser-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (/tmp/hl-gubser-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a100}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{100}$}
\psfrag{a10}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a150}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{150}$}
\psfrag{a15}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{15}$}
\psfrag{a200}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{200}$}
\psfrag{a20}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{20}$}
\psfrag{a250}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{250}$}
\psfrag{a25}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{25}$}
\psfrag{a300}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{300}$}
\psfrag{a30}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{30}$}
\psfrag{a350}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{350}$}
\psfrag{a50}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{50}$}
\psfrag{a5}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{5}$}
\psfrag{Gubser}[bc][bc][\psfragdefaultscale][0]{}
\psfrag{mH}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{\tmh}$}
\psfrag{MHL}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\tilde{M}_{HL}}$}

==> pictures/hl-gubser-scaled-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (/tmp/hl-gubser-scaled-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{a10}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{10}$}
\psfrag{a12}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{12}$}
\psfrag{a14}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{14}$}
\psfrag{a16}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{16}$}
\psfrag{a2}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{2}$}
\psfrag{a40}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{40}$}
\psfrag{a4}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{4}$}
\psfrag{a50}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{50}$}
\psfrag{a60}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{60}$}
\psfrag{a6}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{6}$}
\psfrag{a70}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{70}$}
\psfrag{a80}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{80}$}
\psfrag{a8}[cr][cr][\psfragdefaultscale][0]{$\psfragnumericstyle{8}$}
\psfrag{a90}[tc][tc][\psfragdefaultscale][0]{$\psfragnumericstyle{90}$}
\psfrag{Gubser}[bc][bc][\psfragdefaultscale][0]{}
\psfrag{mH}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{\tmh}$}
\psfrag{MHLmH}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\displaystyle\frac{\tilde{M}_{HL}}{\tmh}}$}

==> pictures/hl-gubser-xmas-compare-lambda100-all-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (hl-gubser-xmas-compare-lambda100-all-psfrag.eps). 
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a0a}[bc][bc][1][0]{$0$}
\psfrag{a10a}[tc][tc][1][0]{$10$}
\psfrag{a15a}[tc][tc][1][0]{$15$}
\psfrag{a1a}[cr][cr][1][0]{$1$}
\psfrag{a20a}[tc][tc][1][0]{$20$}
\psfrag{a25a}[tc][tc][1][0]{$25$}
\psfrag{a2a}[cr][cr][1][0]{$2$}
\psfrag{a30a}[tc][tc][1][0]{$30$}
\psfrag{a3a}[cr][cr][1][0]{$3$}
\psfrag{a4a}[cr][cr][1][0]{$4$}
\psfrag{a5Aa}[cr][cr][1][0]{$5$}
\psfrag{a5a}[tc][tc][1][0]{$5$}
\psfrag{a6a}[cr][cr][1][0]{$6$}
\psfrag{am1MHLmHa}[bc][bc][1][0]{$\frac{M_{\text{HL}}}{m_H}-1$}
\psfrag{amHCLambdaba}[cl][cl][1][0]{$\frac{m_H}{\Lambda _b}$}

==> pictures/limitcycle-psfrag.tex <==
% -- content from the PSfragPrologue option --
% The `auto-ignore' makes arXiv.org ignore this file:
%auto-ignore
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (limitcycle-psfrag.eps). 
\providecommand{\psfragdefaultscale}{1}
\providecommand{\psfragtextstyle}{}
\providecommand{\psfragmathstyle}{}
\providecommand{\psfragnumericstyle}{}
% -- end of PSfragPrologue option --

% psfrag replacement commands
\psfrag{IRlimi}[cl][cl][\psfragdefaultscale][0]{ \acro{IR} limit cycle}
\psfrag{LambdaA}[bc][bc][\psfragdefaultscale][0]{$\psfragmathstyle{\lambda ^j}$}
\psfrag{Lambda}[cl][cl][\psfragdefaultscale][0]{$\psfragmathstyle{\lambda ^i}$}
\psfrag{UVfixe}[cl][cl][\psfragdefaultscale][0]{ \acro{UV} fixed point}

==> pictures/meson-garb-log-psfrag.tex <==
% psfrag replacement commands
\psfrag{a10000}[Br][Br][1][0]{$10^{3}$}
\psfrag{a1000}[tc][tc][1][0]{$10^{3}$}
\psfrag{a1001}[Br][Br][1][0]{$10^{2}$}
\psfrag{a100}[tc][tc][1][0]{$10^{2}$}
\psfrag{a101}[Br][Br][1][0]{$10^{1}$}
\psfrag{a10}[tc][tc][1][0]{$10^{1}$}
\psfrag{a11}[Br][Br][1][0]{$10^{0}$}
\psfrag{a1}[tc][tc][1][0]{$10^{0}$}
\psfrag{a2mPiD}[Bl][Bl][1][0]{$\frac{2\pi\alpha'm_q}{\Lambda}$}
\psfrag{L2MCLa}[bc][bc][1][0]{$\frac{M L^2}{\Lambda}$}
\psfrag{Scaled}[Bc][Bc][1][0]{}

==> pictures/meson-garb-psfrag.tex <==
% psfrag replacement commands
\psfrag{a02}[tc][tc][1][0]{$0.2$}
\psfrag{a04}[tc][tc][1][0]{$0.4$}
\psfrag{a06000}[tc][tc][1][0]{$0.6$}
\psfrag{a08}[tc][tc][1][0]{$0.8$}
\psfrag{a10}[Br][Br][1][0]{$10$}
\psfrag{a15}[Br][Br][1][0]{$15$}
\psfrag{a1}[tc][tc][1][0]{$1$}
\psfrag{a2mPiD}[Bl][Bl][1][0]{$\frac{2\pi\alpha'm_q}{\Lambda}$}
\psfrag{a5}[Br][Br][1][0]{$5$}
\psfrag{L2MCLa}[bc][bc][1][0]{$\frac{M L^2}{\Lambda}$}
\psfrag{Scaled}[Bc][Bc][1][0]{}

==> pictures/meson-ladder-psfrag.tex <==
% psfrag replacement commands
\psfrag{a001}[tc][tc][1][0]{$10^{-2}$}
\psfrag{a01}[tc][tc][1][0]{$10^{-1}$}
\psfrag{a1000}[tc][tc][1][0]{$10^{3}$}
\psfrag{a100}[tc][tc][1][0]{$10^{2}$}
\psfrag{a101}[Br][Br][1][0]{$10$}
\psfrag{a10}[tc][tc][1][0]{$10^{1}$}
\psfrag{a15}[Br][Br][1][0]{$15$}
\psfrag{a1}[tc][tc][1][0]{$10^{0}$}
\psfrag{a20}[Br][Br][1][0]{$20$}
\psfrag{a5}[Br][Br][1][0]{$5$}
\psfrag{CLambd}[Bl][Bl][1][0]{$\frac{\Lambda}{2\pi\alpha'm_q}$}
\psfrag{L2M2mP}[bc][bc][1][0]{$\frac{M L^2}{(2\pi\alpha') m_q}$}
\psfrag{Scaled}[Bc][Bc][1][0]{}

==> styles/keyval.tex <==
%%
%% This is file `keyval.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvkeyval')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2005 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, pst-xkey.tex, pst-xkey.sty, xkveca.cls, xkvecb.cls,
%% xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex, xkvex2.tex,
%% xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, pst-xkey.dtx and xkeyval.dtx.
%%
%%
%% Based on keyval.sty.
%%
\def\XKV@tempa#1{%
\def\KV@@sp@def##1##2{%
  \futurelet\XKV@resa\KV@@sp@d##2\@nil\@nil#1\@nil\relax##1}%
\def\KV@@sp@d{%
  \ifx\XKV@resa\@sptoken
    \expandafter\KV@@sp@b
  \else
    \expandafter\KV@@sp@b\expandafter#1%
  \fi}%
\def\KV@@sp@b#1##1 \@nil{\KV@@sp@c##1}%
  }
\XKV@tempa{ }
\def\KV@@sp@c#1\@nil#2\relax#3{\XKV@toks{#1}\edef#3{\the\XKV@toks}}
\def\KV@do#1,{%
 \ifx\relax#1\@empty\else
  \KV@split#1==\relax
  \expandafter\KV@do\fi}
\def\KV@split#1=#2=#3\relax{%
  \KV@@sp@def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@empty\else
    \expandafter\let\expandafter\XKV@tempc
      \csname\KV@prefix\XKV@tempa\endcsname
    \ifx\XKV@tempc\relax
      \XKV@err{`\XKV@tempa' undefined}%
    \else
      \ifx\@empty#3\@empty
        \KV@default
      \else
        \KV@@sp@def\XKV@tempb{#2}%
        \expandafter\XKV@tempc\expandafter{\XKV@tempb}\relax
      \fi
    \fi
  \fi}
\def\KV@default{%
  \expandafter\let\expandafter\XKV@tempb
    \csname\KV@prefix\XKV@tempa @default\endcsname
  \ifx\XKV@tempb\relax
    \XKV@err{No value specified for key `\XKV@tempa'}%
  \else
    \XKV@tempb\relax
  \fi}
\endinput
%%
%% End of file `keyval.tex'.


==> styles/pst-xkey.tex <==
%%
%% This is file `pst-xkey.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `pxktex')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2005 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, pst-xkey.tex, pst-xkey.sty, xkveca.cls, xkvecb.cls,
%% xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex, xkvex2.tex,
%% xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname PSTXKeyLoaded\endcsname
\let\PSTXKeyLoaded\endinput
\edef\PSTXKeyCatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \let\noexpand\PSTXKeyCatcodes\relax
}
\catcode`\@=11\relax
\ifx\ProvidesFile\@undefined
  \message{2005/02/22 v1.5 PSTricks specialization of xkeyval (HA)}
  \ifx\XKeyValLoaded\endinput\else\input xkeyval \fi
\else
  \ProvidesFile{pst-xkey.tex}
    [2005/02/22 v1.5 PSTricks specialization of xkeyval (HA)]
  \@addtofilelist{pst-xkey.tex}
  \RequirePackage{xkeyval}
\fi
\def\pst@famlist{}
\def\pst@addfams#1{%
  \XKV@for@n{#1}\XKV@tempa{%
    \@expandtwoargs\in@{,\XKV@tempa,}{,\pst@famlist,}%
    \ifin@\else\edef\pst@famlist{\pst@famlist,\XKV@tempa}\fi
  }%
}
\def\psset{%
  \expandafter\@testopt\expandafter\pss@t\expandafter{\pst@famlist}%
}
\def\pss@t[#1]{\setkeys+[psset]{#1}}
\def\@psset#1,\@nil{%
  \edef\XKV@tempa{\noexpand\setkeys+[psset]{\pst@famlist}}%
  \XKV@tempa{#1}%
}
\PSTXKeyCatcodes
\endinput
%%
%% End of file `pst-xkey.tex'.


==> styles/xkeyval.tex <==
%%
%% This is file `xkeyval.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvtex')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2005 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, pst-xkey.tex, pst-xkey.sty, xkveca.cls, xkvecb.cls,
%% xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex, xkvex2.tex,
%% xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname XKeyValLoaded\endcsname
\let\XKeyValLoaded\endinput
\edef\XKVcatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \catcode`\noexpand\=\the\catcode`\=\relax
  \catcode`\noexpand\,\the\catcode`\,\relax
  \catcode`\noexpand\:\the\catcode`\:\relax
  \let\noexpand\XKVcatcodes\relax
}
\catcode`\@11\relax
\catcode`\=12\relax
\catcode`\,12\relax
\catcode`\:12\relax
\newtoks\XKV@toks
\newcount\XKV@depth
\newif\ifXKV@st
\newif\ifXKV@sg
\newif\ifXKV@pl
\newif\ifXKV@knf
\newif\ifXKV@rkv
\newif\ifXKV@inpox
\newif\ifXKV@preset
\let\XKV@rm\@empty
\ifx\ProvidesFile\@undefined
  \message{2005/08/12 v2.5d key=value parser (HA)}
  \input xkvtxhdr
\else
  \ProvidesFile{xkeyval.tex}[2005/08/12 v2.5d key=value parser (HA)]
  \@addtofilelist{xkeyval.tex}
\fi
\long\def\@firstoftwo#1#2{#1}
\long\def\@secondoftwo#1#2{#2}
\long\def\XKV@afterfi#1\fi{\fi#1}
\long\def\XKV@afterelsefi#1\else#2\fi{\fi#1}
\ifx\ifcsname\@undefined\XKV@afterelsefi
  \def\XKV@ifundefined#1{%
    \begingroup\expandafter\expandafter\expandafter\endgroup
      \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\@firstoftwo
    \else
      \expandafter\@secondoftwo
    \fi
  }
\else
  \def\XKV@ifundefined#1{%
    \ifcsname#1\endcsname
      \expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }
\fi
\XKV@ifundefined{ver@keyval.sty}{
  \input keyval
  \expandafter\def\csname ver@keyval.sty\endcsname{1999/03/16}
}{}
\long\def\@ifnextcharacter#1#2#3{%
  \@ifnextchar\bgroup
  {\@ifnextchar{#1}{#2}{#3}}%
  {\@ifncharacter{#1}{#2}{#3}}%
}
\long\def\@ifncharacter#1#2#3#4{%
  \if\string#1\string#4%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {#2}{#3}#4%
}
\long\def\XKV@for@n#1#2#3{%
  \def#2{#1}%
  \ifx#2\@empty
    \XKV@for@break
  \else
    \expandafter\XKV@f@r
  \fi
  #2{#3}#1,\@nil,%
}
\long\def\XKV@f@r#1#2#3,{%
  \def#1{#3}%
  \ifx#1\@nnil
    \expandafter\@gobbletwo
  \else
    #2\expandafter\XKV@f@r
  \fi
  #1{#2}%
}
\long\def\XKV@for@break #1\@nil,{\fi}
\long\def\XKV@for@o#1{\expandafter\XKV@for@n\expandafter{#1}}
\long\def\XKV@for@en#1#2#3{\XKV@f@r#2{#3}#1,\@nil,}
\long\def\XKV@for@eo#1#2#3{%
  \def#2{\XKV@f@r#2{#3}}\expandafter#2#1,\@nil,%
}
\long\def\XKV@whilist#1#2#3\fi#4{%
  #3\expandafter\XKV@wh@list#1,\@nil,\@nil\@@#2#3\fi{#4}{}\fi
}
\long\def\XKV@wh@list#1,#2\@@#3#4\fi#5#6{%
  \def#3{#1}%
  \ifx#3\@nnil
    \def#3{#6}\expandafter\XKV@wh@l@st
  \else
    #4%
      #5\expandafter\expandafter\expandafter\XKV@wh@list
    \else
      \def#3{#6}\expandafter\expandafter\expandafter\XKV@wh@l@st
    \fi
  \fi
  #2\@@#3#4\fi{#5}{#1}%
}
\long\def\XKV@wh@l@st#1\@@#2#3\fi#4#5{}
\def\XKV@addtomacro@n#1#2{%
  \expandafter\def\expandafter#1\expandafter{#1#2}%
}
\def\XKV@addtomacro@o#1#2{%
  \expandafter\expandafter\expandafter\def
    \expandafter\expandafter\expandafter#1\expandafter
    \expandafter\expandafter{\expandafter#1#2}%
}
\def\XKV@addtolist@n#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@n#1{#2}%
  \else
    \XKV@addtomacro@n#1{,#2}%
  \fi
}
\def\XKV@addtolist@o#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@o#1#2%
  \else
    \XKV@addtomacro@o#1{\expandafter,#2}%
  \fi
}
\def\XKV@addtolist@x#1#2{\edef#1{#1\ifx#1\@empty\else,\fi#2}}
\def\@selective@sanitize{\@testopt\@s@lective@sanitize\@M}
\def\@s@lective@sanitize[#1]#2#3{%
  \begingroup
    \count@#1\relax\advance\count@\@ne
    \XKV@toks\expandafter{#3}%
    \def#3{#2}\@onelevel@sanitize#3%
    \edef#3{{#3}{\the\XKV@toks}}%
    \expandafter\@s@l@ctive@sanitize\expandafter#3#3%
  \expandafter\endgroup\expandafter\def\expandafter#3\expandafter{#3}%
}
\def\@s@l@ctive@sanitize#1#2#3{%
  \def\@i{\futurelet\@@tok\@ii}%
  \def\@ii{%
    \expandafter\@iii\meaning\@@tok\relax
    \ifx\@@tok\@s@l@ctive@sanitize
      \let\@@cmd\@gobble
    \else
      \ifx\@@tok\@sptoken
        \XKV@toks\expandafter{#1}\edef#1{\the\XKV@toks\space}%
        \def\@@cmd{\afterassignment\@i\let\@@tok= }%
      \else
        \let\@@cmd\@iv
      \fi
    \fi
    \@@cmd
  }%
  \def\@iii##1##2\relax{\if##1\@backslashchar\let\@@tok\relax\fi}%
  \def\@iv##1{%
    \toks@\expandafter{#1}\XKV@toks{##1}%
    \ifx\@@tok\bgroup
      \advance\count@\m@ne
      \ifnum\count@>\z@
        \begingroup
          \def#1{\expandafter\@s@l@ctive@sanitize
            \csname\string#1\endcsname{#2}}%
          \expandafter#1\expandafter{\the\XKV@toks}%
          \XKV@toks\expandafter\expandafter\expandafter
            {\csname\string#1\endcsname}%
          \edef#1{\noexpand\XKV@toks{\the\XKV@toks}}%
        \expandafter\endgroup#1%
      \fi
      \edef#1{\the\toks@{\the\XKV@toks}}%
      \advance\count@\@ne
      \let\@@cmd\@i
    \else
      \edef#1{\expandafter\string\the\XKV@toks}%
      \expandafter\in@\expandafter{#1}{#2}%
      \edef#1{\the\toks@\ifin@#1\else
              \ifx\@@tok\@sptoken\space\else\the\XKV@toks\fi\fi}%
      \edef\@@cmd{\noexpand\@i\ifx\@@tok\@sptoken\the\XKV@toks\fi}%
    \fi
    \@@cmd
  }%
  \let#1\@empty\@i#3\@s@l@ctive@sanitize
}
\def\XKV@checksanitizea#1#2{%
  \XKV@ch@cksanitize{#1}#2=%
  \ifin@\else\XKV@ch@cksanitize{#1}#2,\fi
  \ifin@\@selective@sanitize[0]{,=}#2\fi
}
\def\XKV@checksanitizeb#1#2{%
  \XKV@ch@cksanitize{#1}#2,%
  \ifin@\@selective@sanitize[0],#2\fi
}
\def\XKV@ch@cksanitize#1#2#3{%
  \def#2{#1}%
  \@onelevel@sanitize#2%
  \@expandtwoargs\in@#3{#2}%
  \ifin@
    \def#2##1#3##2\@nil{%
      \def#2{##2}%
      \ifx#2\@empty\else\in@false\fi
    }%
    #2#1#3\@nil
  \fi
  \def#2{#1}%
}
\def\XKV@sp@deflist#1#2{%
  \let#1\@empty
  \XKV@for@n{#2}\XKV@resa{%
    \expandafter\KV@@sp@def\expandafter\XKV@resa\expandafter{\XKV@resa}%
    \XKV@addtomacro@o#1{\expandafter,\XKV@resa}%
  }%
  \ifx#1\@empty\else
    \def\XKV@resa,##1\@nil{\def#1{##1}}%
    \expandafter\XKV@resa#1\@nil
  \fi
}
\def\XKV@merge#1#2#3{%
  \XKV@checksanitizea{#2}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@pltrue
    #3\XKV@tempa\XKV@tempb
    \let\XKV@tempc#1%
    \let#1\@empty
    \XKV@for@o\XKV@tempc\XKV@tempc{%
      #3\XKV@tempc\XKV@tempd
      \ifx\XKV@tempb\XKV@tempd
        \XKV@plfalse
        \XKV@addtolist@o#1\XKV@tempa
      \else
        \XKV@addtolist@o#1\XKV@tempc
      \fi
    }%
    \ifXKV@pl\XKV@addtolist@o#1\XKV@tempa\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\def\XKV@delete#1#2#3{%
  \XKV@checksanitizeb{#2}\XKV@tempa
  \let\XKV@tempb#1%
  \let#1\@empty
  \XKV@for@o\XKV@tempb\XKV@tempb{%
    #3\XKV@tempb\XKV@tempc
    \@expandtwoargs\in@{,\XKV@tempc,}{,\XKV@tempa,}%
    \ifin@\else\XKV@addtolist@o#1\XKV@tempb\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\def\XKV@warn#1{\message{xkeyval warning: #1}}
\def\XKV@err#1{\errmessage{xkeyval error: #1}}
\def\KV@errx{\XKV@err}
\let\KV@err\KV@errx
\def\XKV@ifstar#1{\@ifnextcharacter*{\@firstoftwo{#1}}}
\def\XKV@ifplus#1{\@ifnextcharacter+{\@firstoftwo{#1}}}
\def\XKV@makepf#1{%
  \KV@@sp@def\XKV@prefix{#1}%
  \def\XKV@resa{XKV}%
  \ifx\XKV@prefix\XKV@resa
    \XKV@err{`XKV' prefix is not allowed}%
    \let\XKV@prefix\@empty
  \else
    \edef\XKV@prefix{\ifx\XKV@prefix\@empty\else\XKV@prefix @\fi}%
  \fi
}
\def\XKV@makehd#1{%
  \expandafter\KV@@sp@def\expandafter\XKV@header\expandafter{#1}%
  \edef\XKV@header{%
    \XKV@prefix\ifx\XKV@header\@empty\else\XKV@header @\fi
  }%
}
\def\XKV@srstate#1#2{%
  \ifx\@empty#2\@empty\advance\XKV@depth\@ne\fi
  \XKV@for@n{XKV@prefix,XKV@fams,XKV@na,ifXKV@st,ifXKV@pl,ifXKV@knf}%
    \XKV@resa{\expandafter\let\csname\XKV@resa#1\expandafter
      \endcsname\csname\XKV@resa#2\endcsname
  }%
  \ifx\@empty#1\@empty\advance\XKV@depth\m@ne\fi
}
\def\XKV@testopta#1{%
  \XKV@ifstar{\XKV@sttrue\XKV@t@stopta{#1}}%
    {\XKV@stfalse\XKV@t@stopta{#1}}%
}
\def\XKV@t@stopta#1{\XKV@ifplus{\XKV@pltrue#1}{\XKV@plfalse#1}}
\def\XKV@testoptb#1{\@testopt{\XKV@t@stoptb#1}{KV}}
\def\XKV@t@stoptb#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@makehd{#3}%
  \KV@@sp@def\XKV@tfam{#3}%
  #1%
}
\def\XKV@testoptc#1{\@testopt{\XKV@t@stoptc#1}{KV}}
\def\XKV@t@stoptc#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@checksanitizeb{#3}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \@testopt#1{}%
}
\def\XKV@testoptd#1#2{%
  \XKV@testoptb{%
    \edef\XKV@tempa{#2\XKV@header}%
    \def\XKV@tempb{\@testopt{\XKV@t@stoptd#1}}%
    \expandafter\XKV@tempb\expandafter{\XKV@tempa}%
  }%
}
\def\XKV@t@stoptd#1[#2]#3{%
  \@ifnextchar[{\XKV@sttrue#1{#2}{#3}}{\XKV@stfalse#1{#2}{#3}[]}%
}
\def\XKV@ifcmd#1#2#3{%
  \def\XKV@@ifcmd##1#2##2##3\@nil##4{%
    \def##4{##2}\ifx##4\@nnil
      \def##4{##1}\expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
  \XKV@@ifcmd#1#2{\@nil}\@nil#3%
}
\def\XKV@getkeyname#1#2{\expandafter\XKV@g@tkeyname#1=\@nil#2}
\def\XKV@g@tkeyname#1=#2\@nil#3{%
  \XKV@ifcmd{#1}\savevalue#3{\XKV@rkvtrue\XKV@sgfalse}{%
    \XKV@ifcmd{#1}\gsavevalue#3%
      {\XKV@rkvtrue\XKV@sgtrue}{\XKV@rkvfalse\XKV@sgfalse}%
  }%
}
\def\XKV@getsg#1#2{%
  \expandafter\XKV@ifcmd\expandafter{#1}\global#2\XKV@sgtrue\XKV@sgfalse
}
\def\XKV@define@default#1#2{%
  \expandafter\def\csname\XKV@header#1@default\expandafter
    \endcsname\expandafter{\csname\XKV@header#1\endcsname{#2}}%
}
\def\define@key{\XKV@testoptb\XKV@define@key}
\def\XKV@define@key#1{%
  \@ifnextchar[{\XKV@d@fine@k@y{#1}}{%
    \expandafter\def\csname\XKV@header#1\endcsname####1%
  }%
}
\def\XKV@d@fine@k@y#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \expandafter\def\csname\XKV@header#1\endcsname##1%
}
\def\define@cmdkey{\XKV@testoptd\XKV@define@cmdkey{cmd}}
\def\XKV@define@cmdkey#1#2[#3]#4{%
  \ifXKV@st\XKV@define@default{#2}{#3}\fi
  \def\XKV@tempa{\expandafter\def\csname\XKV@header#2\endcsname####1}%
  \begingroup\expandafter\endgroup\expandafter\XKV@tempa\expandafter
    {\expandafter\def\csname#1#2\endcsname{##1}#4}%
}
\def\define@cmdkeys{\XKV@testoptd\XKV@define@cmdkeys{cmd}}
\def\XKV@define@cmdkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \edef\XKV@tempa{\noexpand\XKV@define@cmdkey{#1}{\XKV@tempa}}%
    \XKV@tempa[#3]{}%
  }%
}
\def\define@choicekey{\XKV@testopta{\XKV@testoptb\XKV@define@choicekey}}
\def\XKV@define@choicekey#1{\@testopt{\XKV@d@fine@choicekey{#1}}{}}
\def\XKV@d@fine@choicekey#1[#2]#3{%
  \toks@{#2}%
  \XKV@sp@deflist\XKV@tempa{#3}\XKV@toks\expandafter{\XKV@tempa}%
  \@ifnextchar[{\XKV@d@fine@ch@icekey{#1}}{\XKV@d@fine@ch@ic@key{#1}}%
}
\def\XKV@d@fine@ch@icekey#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \XKV@d@fine@ch@ic@key{#1}%
}
\def\XKV@d@fine@ch@ic@key#1{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@ch@ic@k@y
  \else\XKV@afterfi
    \expandafter\XKV@d@f@ne@ch@ic@key
  \fi
  \csname\XKV@header#1\endcsname
}
\def\XKV@d@f@ne@ch@ic@key#1#2{\XKV@d@f@n@@ch@ic@k@y#1{{#2}}}
\def\XKV@d@f@ne@ch@ic@k@y#1#2#3{\XKV@d@f@n@@ch@ic@k@y#1{{#2}{#3}}}
\def\XKV@d@f@n@@ch@ic@k@y#1#2{%
  \edef#1##1{%
    \ifXKV@st\noexpand\XKV@sttrue\else\noexpand\XKV@stfalse\fi
    \ifXKV@pl\noexpand\XKV@pltrue\else\noexpand\XKV@plfalse\fi
    \noexpand\XKV@checkchoice[\the\toks@]{##1}{\the\XKV@toks}%
  }%
  \def\XKV@tempa{\def#1####1}%
  \expandafter\XKV@tempa\expandafter{#1{##1}#2}%
}
\def\define@boolkey{\XKV@t@stopta{\XKV@testoptd\XKV@define@boolkey{}}}
\def\XKV@define@boolkey#1#2[#3]{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@boolkey
  \else\XKV@afterfi
    \expandafter\XKV@d@fine@boolkey
  \fi
  \csname\XKV@header#2\endcsname{#2}{#1#2}{#3}%
}
\def\XKV@d@fine@boolkey#1#2#3#4#5{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}}%
}
\def\XKV@d@f@ne@boolkey#1#2#3#4#5#6{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}{#6}}%
}
\def\XKV@d@f@ne@b@olkey#1#2#3#4#5{%
  \expandafter\newif\csname if#3\endcsname
  \ifXKV@st\XKV@define@default{#2}{#4}\fi
  \ifXKV@pl
    \def#1##1{\XKV@pltrue\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \else
    \def#1##1{\XKV@plfalse\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \fi
}
\def\define@boolkeys{\XKV@plfalse\XKV@testoptd\XKV@define@boolkeys{}}
\def\XKV@define@boolkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \expandafter\XKV@d@fine@boolkeys\expandafter{\XKV@tempa}{#1}{#3}%
  }%
}
\def\XKV@d@fine@boolkeys#1#2#3{%
  \expandafter\XKV@d@f@ne@b@olkey\csname\XKV@header#1\endcsname
    {#1}{#2#1}{#3}{{\csname#2#1\XKV@resa\endcsname}}%
}
\def\XKV@cc{\XKV@testopta{\@testopt\XKV@checkchoice{}}}
\def\XKV@checkchoice[#1]#2#3{%
  \def\XKV@tempa{#1}%
  \ifXKV@st\lowercase{\fi
  \ifx\XKV@tempa\@empty
    \def\XKV@tempa{\XKV@ch@ckch@ice\@nil{#2}{#3}}%
  \else
    \def\XKV@tempa{\XKV@ch@ckchoice#1\@nil{#2}{#3}}%
  \fi
  \ifXKV@st}\fi\XKV@tempa
}
\def\XKV@ch@ckchoice#1#2\@nil#3#4{%
  \def\XKV@tempa{#2}%
  \ifx\XKV@tempa\@empty\XKV@afterelsefi
    \XKV@ch@ckch@ice#1{#3}{#4}%
  \else\XKV@afterfi
    \XKV@@ch@ckchoice#1#2{#3}{#4}%
  \fi
}
\def\XKV@ch@ckch@ice#1#2#3{%
  \def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@nnil\let\XKV@tempa\@empty\else
    \def\XKV@tempa{\def#1{#2}}%
  \fi
  \in@{,#2,}{,#3,}%
  \ifin@
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@firstoftwo
    \else
      \XKV@addtomacro@n\XKV@tempa\@firstofone
    \fi
  \else
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@secondoftwo
    \else
      \XKV@toks{#2}%
      \XKV@err{value `\the\XKV@toks' is not allowed}%
      \XKV@addtomacro@n\XKV@tempa\@gobble
    \fi
  \fi
  \XKV@tempa
}
\def\XKV@@ch@ckchoice#1#2#3#4{%
  \edef\XKV@tempa{\the\count@}\count@\z@
  \def\XKV@tempb{#3}%
  \def\XKV@tempc##1,{%
    \def#1{##1}%
    \ifx#1\@nnil
      \def#1{#3}\def#2{-1}\count@\XKV@tempa
      \ifXKV@pl
        \let\XKV@tempd\@secondoftwo
      \else
        \XKV@toks{#3}%
        \XKV@err{value `\the\XKV@toks' is not allowed}%
        \let\XKV@tempd\@gobble
      \fi
    \else
      \ifx#1\XKV@tempb
        \edef#2{\the\count@}\count@\XKV@tempa
        \ifXKV@pl
          \let\XKV@tempd\XKV@@ch@ckch@ice
        \else
          \let\XKV@tempd\XKV@@ch@ckch@ic@
        \fi
      \else
        \advance\count@\@ne
        \let\XKV@tempd\XKV@tempc
      \fi
    \fi
    \XKV@tempd
  }%
  \XKV@tempc#4,\@nil,%
}
\def\XKV@@ch@ckch@ice#1\@nil,{\@firstoftwo}
\def\XKV@@ch@ckch@ic@#1\@nil,{\@firstofone}
\def\key@ifundefined{\@testopt\XKV@key@ifundefined{KV}}
\def\XKV@key@ifundefined[#1]#2{%
  \XKV@makepf{#1}%
  \XKV@checksanitizeb{#2}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \XKV@key@if@ndefined
}
\def\XKV@key@if@ndefined#1{%
  \XKV@knftrue
  \KV@@sp@def\XKV@tkey{#1}%
  \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{\XKV@header\XKV@tkey}{}{\XKV@knffalse}%
  }%
  \ifXKV@knf
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\def\disable@keys{\XKV@testoptb\XKV@disable@keys}
\def\XKV@disable@keys#1{%
  \XKV@checksanitizeb{#1}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@ifundefined{\XKV@header\XKV@tempa}{%
      \XKV@err{key `\XKV@tempa' undefined}%
    }{%
      \edef\XKV@tempb{%
        \noexpand\XKV@warn{key `\XKV@tempa' has been disabled}%
      }%
      \XKV@ifundefined{\XKV@header\XKV@tempa @default}{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}}%
      }{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}[]}%
      }%
      \expandafter\XKV@tempc\expandafter{\XKV@tempb}%
    }%
  }%
}
\def\presetkeys{\XKV@stfalse\XKV@testoptb\XKV@presetkeys}
\def\gpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@presetkeys}
\def\XKV@presetkeys#1#2{%
  \XKV@pr@setkeys{#1}{preseth}%
  \XKV@pr@setkeys{#2}{presett}%
}
\def\XKV@pr@setkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@checksanitizea{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname
      XKV@\XKV@header#2\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\delpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@delpresetkeys}
\def\gdelpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@delpresetkeys}
\def\XKV@delpresetkeys#1#2{%
  \XKV@d@lpresetkeys{#1}{preseth}%
  \XKV@d@lpresetkeys{#2}{presett}%
}
\def\XKV@d@lpresetkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\unpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@unpresetkeys}
\def\gunpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@unpresetkeys}
\def\XKV@unpresetkeys{%
  \XKV@ifundefined{XKV@\XKV@header preseth}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header preseth\endcsname\@undefined
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header presett\endcsname\@undefined
  }%
}
\def\savekeys{\XKV@stfalse\XKV@testoptb\XKV@savekeys}
\def\gsavekeys{\XKV@sttrue\XKV@testoptb\XKV@savekeys}
\def\XKV@savekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@checksanitizeb{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname XKV@%
      \XKV@header save\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\delsavekeys{\XKV@stfalse\XKV@testoptb\XKV@delsavekeys}
\def\gdelsavekeys{\XKV@sttrue\XKV@testoptb\XKV@delsavekeys}
\def\XKV@delsavekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\unsavekeys{\XKV@stfalse\XKV@testoptb\XKV@unsavekeys}
\def\gunsavekeys{\XKV@sttrue\XKV@testoptb\XKV@unsavekeys}
\def\XKV@unsavekeys{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header save\endcsname\@undefined
  }%
}
\def\setkeys{\XKV@testopta{\XKV@testoptc\XKV@setkeys}}
\def\XKV@setkeys[#1]#2{%
  \XKV@checksanitizea{#2}\XKV@resb
  \let\XKV@naa\@empty
  \XKV@for@o\XKV@resb\XKV@tempa{%
    \expandafter\XKV@g@tkeyname\XKV@tempa=\@nil\XKV@tempa
    \XKV@addtolist@x\XKV@naa\XKV@tempa
  }%
  \let\XKV@rm\@empty
  \XKV@usepresetkeys{#1}{preseth}%
  \expandafter\XKV@s@tkeys\expandafter{\XKV@resb}{#1}%
  \XKV@usepresetkeys{#1}{presett}%
}
\def\XKV@usepresetkeys#1#2{%
  \XKV@presettrue
  \XKV@for@eo\XKV@fams\XKV@tfam{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{XKV@\XKV@header#2}{}{%
      \XKV@toks\expandafter\expandafter\expandafter
        {\csname XKV@\XKV@header#2\endcsname}%
      \@expandtwoargs\XKV@s@tkeys{\the\XKV@toks}%
        {\XKV@naa\ifx\XKV@naa\@empty\else,\fi#1}%
    }%
  }%
  \XKV@presetfalse
}
\def\XKV@s@tkeys#1#2{%
  \XKV@sp@deflist\XKV@na{#2}%
  \XKV@for@n{#1}\CurrentOption{%
    \expandafter\XKV@s@tk@ys\CurrentOption==\@nil
  }%
}
\def\XKV@s@tk@ys#1=#2=#3\@nil{%
  \XKV@g@tkeyname#1=\@nil\XKV@tkey
  \expandafter\KV@@sp@def\expandafter\XKV@tkey\expandafter{\XKV@tkey}%
  \ifx\XKV@tkey\@empty
    \XKV@toks{#2}%
    \ifcat$\the\XKV@toks$\else
      \XKV@err{no key specified for value `\the\XKV@toks'}%
    \fi
  \else
    \@expandtwoargs\in@{,\XKV@tkey,}{,\XKV@na,}%
    \ifin@\else
      \XKV@knftrue
      \KV@@sp@def\XKV@tempa{#2}%
      \ifXKV@preset\XKV@s@tk@ys@{#3}\else
        \ifXKV@pl
          \XKV@for@eo\XKV@fams\XKV@tfam{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \else
          \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \fi
      \fi
      \ifXKV@knf
        \ifXKV@inpox
          \ifx\XKV@doxs\relax
            \ifx\@currext\@clsextension\else
              \let\CurrentOption\XKV@tkey\@unknownoptionerror
            \fi
          \else\XKV@doxs\fi
        \else
          \ifXKV@st
            \global\XKV@addtolist@o\XKV@rm\CurrentOption
          \else
            \XKV@err{`\XKV@tkey' undefined in families `\XKV@fams'}%
          \fi
        \fi
      \else
        \ifXKV@inpox\ifx\XKV@testclass\XKV@documentclass
          \expandafter\XKV@useoption\expandafter{\CurrentOption}%
        \fi\fi
      \fi
    \fi
  \fi
}
\def\XKV@s@tk@ys@#1{%
  \XKV@ifundefined{\XKV@header\XKV@tkey}{}{%
    \XKV@knffalse
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter{\XKV@tempa}%
    \ifx\@empty#1\@empty\XKV@afterelsefi
      \XKV@ifundefined{\XKV@header\XKV@tkey @default}{%
        \XKV@err{no value specified for key `\XKV@tkey'}%
      }{%
        \expandafter\expandafter\expandafter\XKV@default
          \csname\XKV@header\XKV@tkey @default\endcsname\@nil
      }%
    \else\XKV@afterfi
      \XKV@srstate{@\romannumeral\XKV@depth}{}%
      \csname\XKV@header\XKV@tkey\expandafter
        \endcsname\expandafter{\XKV@tempa}\relax
      \XKV@srstate{}{@\romannumeral\XKV@depth}%
    \fi
  }%
}
\def\XKV@testsavekey#1#2{%
  \ifXKV@rkv\else
    \XKV@for@o#1\XKV@resa{%
      \expandafter\XKV@ifcmd\expandafter{\XKV@resa}\global\XKV@resa{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgtrue
        \fi
      }{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgfalse
        \fi
      }%
    }%
  \fi
}
\def\XKV@replacepointers#1{%
  \let\XKV@tempa\@empty
  \let\XKV@resa\@empty
  \XKV@r@placepointers#1\usevalue\@nil
}
\def\XKV@r@placepointers#1\usevalue#2{%
  \XKV@addtomacro@n\XKV@tempa{#1}%
  \def\XKV@tempb{#2}%
  \ifx\XKV@tempb\@nnil\else\XKV@afterfi
    \XKV@ifundefined{XKV@\XKV@header#2@value}{%
      \XKV@err{no value recorded for key `#2'; ignored}%
      \XKV@r@placepointers
    }{%
      \@expandtwoargs\in@{,#2,}{,\XKV@resa,}%
      \ifin@\XKV@afterelsefi
        \XKV@err{back linking pointers; pointer replacement canceled}%
      \else\XKV@afterfi
        \XKV@addtolist@x\XKV@resa{#2}%
        \expandafter\expandafter\expandafter\XKV@r@placepointers
          \csname XKV@\XKV@header#2@value\endcsname
      \fi
    }%
  \fi
}
\def\XKV@default#1#2\@nil{%
  \expandafter\edef\expandafter\XKV@tempa
    \expandafter{\expandafter\@gobble\string#1}%
  \edef\XKV@tempb{\XKV@header\XKV@tkey}%
  \@onelevel@sanitize\XKV@tempb
  \ifx\XKV@tempa\XKV@tempb
    \begingroup
      \expandafter\def\csname\XKV@header\XKV@tkey\endcsname##1{%
        \gdef\XKV@tempa{##1}%
      }%
      \csname\XKV@header\XKV@tkey @default\endcsname
    \endgroup
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter
      {\XKV@tempa}\XKV@afterelsefi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \expandafter#1\expandafter{\XKV@tempa}\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \else\XKV@afterfi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \csname\XKV@header\XKV@tkey @default\endcsname\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \fi
}
\def\setrmkeys{\XKV@testopta{\XKV@testoptc\XKV@setrmkeys}}
\def\XKV@setrmkeys[#1]{%
  \def\XKV@tempa{\XKV@setkeys[#1]}%
  \expandafter\XKV@tempa\expandafter{\XKV@rm}%
}
\XKVcatcodes
\endinput
%%
%% End of file `xkeyval.tex'.


==> styles/xkvtxhdr.tex <==
%%
%% This is file `xkvtxhdr.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvheader')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2005 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, pst-xkey.tex, pst-xkey.sty, xkveca.cls, xkvecb.cls,
%% xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex, xkvex2.tex,
%% xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, pst-xkey.dtx and xkeyval.dtx.
%%
%%
%% Taken from latex.ltx.
%%
\message{2005/02/22 v1.1 xkeyval TeX header (HA)}
\def\@nnil{\@nil}
\def\@empty{}
\def\newif#1{%
  \count@\escapechar \escapechar\m@ne
    \let#1\iffalse
    \@if#1\iftrue
    \@if#1\iffalse
  \escapechar\count@}
\def\@if#1#2{%
  \expandafter\def\csname\expandafter\@gobbletwo\string#1%
                    \expandafter\@gobbletwo\string#2\endcsname
                       {\let#1#2}}
\long\def\@ifnextchar#1#2#3{%
  \let\reserved@d=#1%
  \def\reserved@a{#2}%
  \def\reserved@b{#3}%
  \futurelet\@let@token\@ifnch}
\def\@ifnch{%
  \ifx\@let@token\@sptoken
    \let\reserved@c\@xifnch
  \else
    \ifx\@let@token\reserved@d
      \let\reserved@c\reserved@a
    \else
      \let\reserved@c\reserved@b
    \fi
  \fi
  \reserved@c}
\def\:{\let\@sptoken= } \:  % this makes \@sptoken a space token
\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@token\@ifnch}
\let\kernel@ifnextchar\@ifnextchar
\long\def\@testopt#1#2{%
  \kernel@ifnextchar[{#1}{#1[{#2}]}}
\long\def\@firstofone#1{#1}
\long\def \@gobble #1{}
\long\def \@gobbletwo #1#2{}
\def\@expandtwoargs#1#2#3{%
\edef\reserved@a{\noexpand#1{#2}{#3}}\reserved@a}
\edef\@backslashchar{\expandafter\@gobble\string\\}
\newif\ifin@
\def\in@#1#2{%
 \def\in@@##1#1##2##3\in@@{%
  \ifx\in@##2\in@false\else\in@true\fi}%
 \in@@#2#1\in@\in@@}
\def\strip@prefix#1>{}
\def \@onelevel@sanitize #1{%
  \edef #1{\expandafter\strip@prefix
           \meaning #1}%
}
\endinput
%%
%% End of file `xkvtxhdr.tex'.

